Threshold Logical Clocks for Asynchronous Distributed Coordination and Consensus

Consensus protocols for asynchronous networks are usually complex and inefficient, leading practical systems to rely on synchronous protocols. This paper attempts to simplify asynchronous consensus by building atop a novel threshold logical clock abstraction, which enables upper layers to operate as if on a synchronous network. This approach yields an asynchronous consensus protocol for fail-stop nodes that may be simpler and more robust than Paxos and its leader-based variants, requiring no common coins and achieving consensus in a constant expected number of rounds. The same approach can be strengthened against Byzantine failures by building on well-established techniques such as tamper-evident logging and gossip, accountable state machines, threshold signatures and witness cosigning, and verifiable secret sharing. This combination of existing abstractions and threshold logical clocks yields a modular, cleanly-layered approach to building practical and efficient Byzantine consensus, distributed key generation, time, timestamping, and randomness beacons, and other critical services.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -version | egrep -q '201[678]' && echo '\lstloadlanguages{Go,Promela} only works in TexLive 2019 and after' && exit 1 || true
	latexmk -pdf $<

fast:
	pdflatex $(FILE)

allx:
	pdflatex $(FILE)
	bibtex $(FILE)
	pdflatex $(FILE)
	pdflatex $(FILE)


clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d


==> claims.tex <==
\section{Draft Patent Application Claims}

On threshold logical clocks (TLC):
\begin{itemize}
\item	A threshold logical clock (TLC) layer as a substrate
	providing a communication-driven, timeout-free notion of time
	atop an asynchronous network
	to simplify and pace higher-level distributed protocols,
	ensuring that coordinated nodes advance together in lock-step
	(``quasi-synchronously'')
	as quickly as communication over the underlying network permits.
	(Section~\ref{sec:tlc})
\item	A threshold logical clock incorporating
	threshold witnessing~\cite{syta16keeping}
	as a way to ensure proactively that a substantial fraction
	(\eg, a majority or supermajority) of messages broadcast
	at each logical time-step have reached other nodes
	by the end of that time-step,
	and as a way to allow nodes to determine
	which subset(s) of messages have propagated in this way.
	(Section~\ref{sec:tlc:wit})
\item	The enforcement of causally-ordered message delivery in TLC,
	using mechanisms such as vector clocks~\cite{fischer82sacrificing,liskov86highly,mattern89virtual,fidge91logical},
	to ensure that broadcasts by all nodes are delivered
	in causally consistent order to other nodes,
	thereby simplifying the reasoning about information propagation
	in quasi-synchronous protocols building atop TLC.
	(Section~\ref{sec:tlc:causal})
\item	The delineation of real-world time into periods
	according to the moment a {\em majority} of participating TLC nodes
	reach successive logical time steps,
	in order to simplify further protocols built atop TLC,
	both by constraining the earliest time
	any message labeled with a time step $s$ 
	can have been sent (\ie, not before real time period $s$ started),
	and by constraining the latest time
	any received message labeled $s$ can have been formulated
	(\ie, not after real time period $s$ ended).
	(Section~\ref{sec:tlc:periods})
\item	The use of TLC as an automatic reliable broadcast protocol
	ensuring that all messages sent and threshold witnessed
	during any step $s$
	will be seen by {\em all} participating nodes by step $s+2$,
	provided the message and witnessing thresholds are majoritarian
	($>n/2$).
	(Section~\ref{sec:tlc:broadcast})
\end{itemize}

Basic services built on logical clocks:
\begin{itemize}
\item	The use of TLC to build an asynchronous network time service
	for trustworthy clock initialization and synchronization
	(Section~\ref{sec:app:time:sync}).
\item	The use of TLC to build a distributed trusted timestamping service
	enabling clients to prove that a specific document or other data
	existed in original, unmodified form at a specific historical time
	(Section~\ref{sec:app:time:stamp}).
\item	The use of TLC to build an encrypted time vault or time capsule service
	enabling clients to encrypt data so as to be decryptable
	only att a specific future time
	(Section~\ref{sec:app:time:vault}).
\item	The use of TLC to build  an asynchronous public randomness beacon
	that transparently publishes unpredictable, unbiasable random numbers
	as frequently as group configuration and network connectivity permits
	(Section~\ref{sec:app:random}).
\end{itemize}

On building consensus algorithms (``que sera consensus'' or QSC)
atop the abstraction of threshold logical clocks:
\begin{itemize}
\item	The use of TLC to build an asynchronous consensus protocol
	(Section~\ref{sec:cons}).

\item	An asynchronous consensus protocol built atop TLC
	in which every participating node proposes a message
	in the first time step of each round ($s+0$),
	waits a fixed number of TLC time steps,
	then uses history information recorded and exchanged
	between nodes by TLC to determine the result of consensus.

\item	An asynchronous consensus protocol in which each participating node
	maintains an independent possible history,
	represented by a tamper-evident log or blockchain,
	that grows by one record each TLC time-step
	(Section~\ref{sec:cons:histories}).

\item	An asynchronous consensus protocol in which each node,
	at certain TLC time steps,
	chooses to adopt another randomly-chosen node's history or blockchain
	in place of its own,
	yielding in a form of genetic consensus over time while paced by TLC
	(Section~\ref{sec:cons:genetic}).

\item	An asynchronous consensus protocol in which
	each node chooses a random number to attach to its proposal,
	which serves as an artificial ``genetic fitness'' metric
	in that other nodes choose the most fit proposal they are aware of
	to build on in the next round to accelerate genetic consensus
	(Section~\ref{sec:cons:fitness}).

\item	An asynchronous consensus protocol in which
	each node chooses protocols to build on in the next round
	only from those it deems {\em eligible},
	by virtue of having been {\em confirmed} or threshold witnessed
	and thus confirmed to have propagated to a majority of nodes
	(Section~\ref{sec:cons:celebrity}).
	\xxx{ important to contrast this somewhere with
		asynchronous consensus protocols requiring a common coin,
		e.g., VABA etc.  Probably in Related Work. }

\item	An asynchronous consensus protocol in which all nodes
	wait two TLC time-steps after broadcasting their proposals,
	so that all {\em confirmed} proposals
	that were threshold witnessed in the first step (by $s+1$)
	will be known to {\em all} nodes by the end of the second step ($s+2$)
	(Section~\ref{sec:cons:universal}).

\item	An asynchronous consensus protocol in which each node tests
	whether a proposal has been {\em doubly confirmed} or {\em reconfirmed},
	so that it knows that such a proposal's confirmed status
	will have propagated to {\em all} nodes by the third TLC step ($s+3$)
	(Section~\ref{sec:cons:paparazzi}).

\item	An asynchronous consensus protocol in which each node determines,
	via analysis of the round's history exchanged between nodes by TLC,
	in which consensus rounds all nodes will finally choose the same
	best eligible (confirmed) proposal
	(Section~\ref{sec:cons:predict}).

\item	An asynchronous consensus protocol ensuring that an adversarial network
	cannot learn the genetic fitness lottery tickets
	associated with proposals before the consensus round completes
	(Section~\ref{sec:cons:adversary}).

\item	\xxx{ byzantine, pipelining, etc. }
\end{itemize}

On protecting threshold logical clocks and consensus protocols built on it
against Byzantine node behavior:

\begin{itemize}
\item	A threshold logical clock protocol
	in which each node maintains a local tamper-evident log,
	in which each entry is digitally signed by the node
	and linked to prior entries via cryptographic hashes,
	to enable other participating nodes to replay and validate
	the node's decisions and actions affecting the group
	(Section~\ref{sec:byz:log}).

\item	A threshold logical clock protocol
	in which each node deterministically replays other nodes' decisions,
	based on the causal history leading up to that decision
	as recorded in that and other nodes' logs,
	to ensure that the verified node correctly implemented
	both the threshold logical clocks logic
	and any deterministically verificable state machine logic
	of protocols built atop the TLC layer
	(Section~\ref{sec:byz:expose}).

\item	A  threshold logical clock protocol
	in which each node uses cryptographic hashes
	to gossip and verify with other nodes that every node
	digitally signs only one message for a given sequence number,
	and if a violatin of this is ever discovered (equivocation),
	the correct nodes expose and gossip proofs of this misbehavior
	(Section~\ref{sec:byz:equiv}).

\item	A threshold logical clock protocol
	in which correct nodes use tamper-evident logging and verification
	to ensure that all other nodes advance their logical clocks correctly,
	and never advance them too quickly  or slowly or turn them back
	(Section~\ref{sec:byz:time-progress}).

\item	A  threshold logical clock protocol designed for a threat model
	that takes two independent configuration parameters,
	$f_a$ describing the maximum number of nodes
	that might be unavailable or unreachable,
	and $f_c$ describing the maximum number of nodes
	that might be corrupt and maliciously colluding
	(Section~\ref{sec:byz:maj}).

\item	A threshold logical clock protocol
	that uses threshold witness cosigning to protect correct nodes
	against equivocation immediately and proactively,
	and not just eventually,
	provided the witness threshold satisifies the constraints
	${n+f_c \over 2} < t_w \le n-f_a$
	and nodes depend only on witness cosigned messages
	to be non-equivocating
	(Section~\ref{sec:byz:wit}).

\item	A threshold logical clock protocol
	that uses logging and verification to ensure that corrupt nodes
	cannot produce a message for a time step $s+1$ or later
	that correct nodes will accept,
	before a majority of correct nodes have reached step $s$
	and global time period $s$ has begun,
	provided the message threshold satisifies the constraints
        ${n+f_c \over 2} < t_m \le n-f_a$
	(Section~\ref{sec:byz:periods}).

\item	A threshold logical clock protocol
	that uses logging and verification to ensure that corrupt nodes
	cannot formulate a new message for a time step $s$ or before
	and get it threshold witnessed in a way correct nodes will accept,
	after a majority of correct nodes have reached step $s+1$
	and global time period $s+1$ has begun,
	provided the witness threshold satisifies the constraints
        ${n+f_c \over 2} < t_w \le n-f_a$
	(Section~\ref{sec:byz:periods}).

\item	A threshold logical clock protocol
	that uses logging and verification to ensure that corrupt nodes
	cannot violate the guarantee that any message threshold witnessed
	at a given time step $s$ will be known to {\em all} nodes --
	and will appear in the causal histories of all nodes,
	even corrupt nodes producing valid logs,
	by the time those nodes reach step $s+2$
	(Section~\ref{sec:byz:bcast}).

\item	A Byzantine consensus protocol that builds on
	a Byzantine-protected threshold logical protocol such as that above
	(Section~\ref{sec:byz:cons}).

\item	A Byzantine consensus protocol that leverages
	the logging, deterministic replay, and verification mechanisms
	in the threshold logical clocks layer
	to protect the core logic of the Byzantine consensus protocol as well
	(Section~\ref{sec:byz:cons-logic}).

\item	A Byzantine consensus protocol that builds on threshold logical clocks
	and that associates genetic fitness lottery tickets with proposals
	so that no one, including the node making the proposal,
	can predict or bias the lottery ticket value before the round completes
	(Section~\ref{sec:byz:tickets}).

\item	A Byzantine consensus protocol bhat builds on threshold logical clocks
	and generates lottery tickets each round using a
	joint publicly verifiable secret sharing (PVSS) scheme
	to ensure that each proposer chooses its ticket fairly
	in a verifiably unpredictable and unbiased fashion,
	using a combination of secrets dealt by at least $f_c+1$ nodes
	to ensure that at least one of those secrets is from a correct node
	(Section~\ref{sec:byz:pvss}).
\end{itemize}

On building asynchronous distributed key generation (DKG)
atop the abstraction of threshold logical clocks:
\begin{itemize}
\item	A distributed key generation (DKG) protocol
	that builds on threshold logical clocks
	to generate a threshold-secret-shared public/private keypair,
	such that no one can learn the composite private key
	but a threshold of group members can coordinate
	to use the shared private key jointly
	for a variety of cryptographic operations and applications
	(Section~\ref{sec:dkg}).

\item	A distributed key generation protocol
	built atop threshold logical clocks
	in which each node deals a matrix of verifiable threshold secret shares
	such that any correct node that receives an incorrect share in a deal
	can recover the correct share from recovery shares
	verified correct by a threshold of correct nodes
	(Section~\ref{sec:dkg:qsdkg}).
\end{itemize}


